uMedSum: A Unified Framework for Advancing Medical Abstractive Summarization

Medical abstractive summarization faces the challenge of balancing faithfulness and informativeness. Current methods often sacrifice key information for faithfulness or introduce confabulations when prioritizing informativeness. While recent advancements in techniques like in-context learning (ICL) and fine-tuning have improved medical summarization, they often overlook crucial aspects such as faithfulness and informativeness without considering advanced methods like model reasoning and self-improvement. Moreover, the field lacks a unified benchmark, hindering systematic evaluation due to varied metrics and datasets. This paper addresses these gaps by presenting a comprehensive benchmark of six advanced abstractive summarization methods across three diverse datasets using five standardized metrics. Building on these findings, we propose uMedSum, a modular hybrid summarization framework that introduces novel approaches for sequential confabulation removal followed by key missing information addition, ensuring both faithfulness and informativeness. Our work improves upon previous GPT-4-based state-of-the-art (SOTA) medical summarization methods, significantly outperforming them in both quantitative metrics and qualitative domain expert evaluations. Notably, we achieve an average relative performance improvement of 11.8% in reference-free metrics over the previous SOTA. Doctors prefer uMedSum's summaries 6 times more than previous SOTA in difficult cases where there are chances of confabulations or missing information. These results highlight uMedSum's effectiveness and generalizability across various datasets and metrics, marking a significant advancement in medical summarization.

==> full_methodology.tex <==
\section{\frameworkname{}: A Pipeline for Faithful and Comprehensive Medical Summarisation}
% \begin{enumerate}
%     \item Show your architecture and describe it briefly
%     \item Explain the general basic idea in one or two paragraphs 
%     \item Discuss in detail the main/new components in your method
%     \item Show and then summarise the whole algorithm 
% \end{enumerate}

% \subsection{\frameworkname{} Pipeline Overview}
% This pipeline is a hybrid approach that integrates both abstractive and extractive summarization techniques to overcome the limitations of each method when used in isolation.

The \frameworkname{} pipeline is designed to produce high-quality, faithful, and comprehensive medical summaries through a three-stage process, visualised in Figure \ref{fig:main-framework}: Initial Summary Generation, Confabulation Detection and Removal, and Missing Information Generation. Each stage of \frameworkname{} is a self-contained module that can be updated and optimized independently, offering flexible and robust usage with minimal additional computational resources required. The modularity of the pipeline enables a plug-and-play approach to work seamlessly with both open and closed-source models during inference. 

% Our approach consists of three independent stages, visualised in Figure~x: We produce a high quality initial summary in Stage I; Stage II detects and removes confabulated information, by identifying sentences that are not entailed by the input; In Stage III, we add potentially missing information, by identifying key phrases and sentences in the input. The resulting summary is then re-arranged to generate a fluent, cohesive summary. We choose a pipelined approach over an end-to-end architecture, in order to be able to augment the faithfulness of any summarization technique. 

\subsection{Stage 1: Initial Summary Generation}
%
% Medical abstractive summarization is an inherently challenging task, balancing the need for concise, readable summaries with the necessity of maintaining factual accuracy and comprehensive coverage. 
\textbf{Background and Assumptions.} 
To address the lack of a systematic benchmark for summarisation methods in medical summarisation, Stage 1 of the \frameworkname{} first benchmarks the most effective summarization techniques. 
% This is done by evaluating \textbf{four} open-source and proprietary large language models (LLMs), including both domain specific and general purpose models, across \textbf{three} biomedical datasets. We employ a combination of \textbf{two} reference-based and \textbf{three} reference-free metrics to assess the quality, faithfulness and comprehensiveness of summaries. 
The combination of best performing methods and models are then selected for further evaluation using all stages of \frameworkname{}.

\textbf{Benchmark and Evaluation Details.} 
% The novelty of Stage 1 lies in its comprehensive evaluation of summarization techniques, employing a combination of four advanced LLMs, 3 diverse biomedical summarisation datasets and evaluated on a combination of two reference based and three reference free summaries.  

% Specifically, we benchmark the performance of \textbf{four models}: LLaMA3 (8B) \cite{meta2024introducing}, Gemma (7B) \cite{team2024gemma}, Meditron (7B) \cite{chen2023meditron70b, epfmedtrn}, and GPT-4 \cite{achiam2023gpt}. These models are evaluated on three biomedical datasets for summarization tasks: MIMIC III for Radiology Report Summarization \cite{johnson2016mimic}, Me QSum for Patient Question Summarization \cite{abacha2019summarization}, and ACI-Bench for doctor-patient dialogue summarization \cite{yim2023aci}. These provide a diverse range of biomedical summarization task settings, with varying document lengths, requirement for background knowledge as well as the need for domain-specific vocabulary and understanding. This diversity allows for a comprehensive evaluation of the models' ability to handle different types of summarization tasks within the biomedical field, each presenting unique challenges in terms of information extraction, summarization accuracy, and relevance. As suggested in previous works by \cite{maynez-etal-2020-faithfulness}, reference based metrics by themselves are not a good measure for evaluating faithfulness and factuality in abstractive summarization tasks, and should be combined with reference free metrics. We thus make use of two reference based techniques, ROUGE-LSum \cite{lin2004rouge} and BERTScore \cite{zhang2019bertscore}, in combination with three reference free metrics, SummaC \cite{laban2022summac}, QuestEval \cite{scialom2021questeval} and Entailment Scores \cite{liu2024hit} for purposes of our evaluation. Let \( S_i \) represent the summary generated by the \( i \)-th summarization technique. The quality of this summary is evaluated using a set of metrics \( M_j \), where \( j \) denotes the specific metric used (e.g., ROUGE-L, BERTScore, SummaC). The score for a given metric \( M_j \) applied to a summary \( S_i \) is denoted as \( M_j(S_i) \).

To identify the best-performing techniques, we first benchmark four summarization methods: Standard Prompting (baseline), Element-aware Summarization with Large Language Models \cite{wang2023element}, Chain of Density \cite{addams2023sparse}, and Hierarchical Summarization \cite{chang2023booookscore}. Each of these techniques come with their specific benefits and downsides. For example, Element-aware Summarization improves content relevance by focusing on (domain) specific elements within the text, leading to more targeted and informative summaries. Chain of Density creates summaries which are information dense at the cost of readability. Hierarchical Summarization has proven to combat the issues of “lost-in-the-middle” in long context summarization \cite{ravaut2023context}.  We then combine the best-performing summarization methods with task adaptation strategies, focusing on In-Context Learning, which has been shown to outperform QLoRA for the same tasks \cite{van2024adapted}. This stage sets the foundation for the subsequent stages by ensuring that the initial summary is of the highest possible quality.

% The final evaluation score for a summary \( S_i \) generated by a specific method is determined by aggregating its rank across all metrics:

% \[
% \text{Rank}_i = \sum_{j=1}^{n} \text{Rank}(M_j(S_i))
% \]

% where \(\text{Rank}(M_j(S_i))\) is the rank of the method based on metric \( M_j \), and \( n \) is the total number of metrics used. The method with the lowest \(\text{Rank}_i\) is considered the most effective.


\subsection{Stage 2: Confabulation Removal (Faithfulness)}

The \frameworkname{} pipeline takes a novel approach by repurposing Natural Language Inference (NLI) models to not just evaluate factuality of generates summaries, but for directly detecting and removing discrete confabulated information from generated summaries during decoding. This approach differs from existing methods, which typically focus on sentence-level entailment or entity-based splitting \cite{lei2023chain}, by introducing a more granular decomposition based on atomic facts \cite{thirukovalluru2024atomic, nawrath2024role, stacey2023logical}.
%Stage 2 introduces a systematic confabulation removal technique that utilizes NLI models for reference-free detection and removal of confabulated information. We
Specifically, propose a two-step process: (1) summary decomposition into smaller, manageable units, and (2) pairwise NLI-based confabulation detection and removal. 

% Need to do citations from here
\textbf{Summary Decomposition.} We begin by decomposing the summary generated in Stage 1 into smaller units called Summary Content Units (SCUs) \citep{nawrath2024role} or Decomposed Summary Units (DSUs). We propose \textit{Recursive Threshold-based Text Segmentation} to further split sentences into clause-level atomic facts. Unlike previous works that stop at sentence-level decomposition or rely on entity-based splitting for further decomposition \cite{lei2023chain}, our approach aims to create self-contained units that encapsulate atomic facts. Atomic facts encapsulate the smallest meaningful statements that can stand alone as true or false propositions. This aligns well with the nature of NLI, where the goal is to determine the logical relationship (e.g., entailment, contradiction, or neutrality) between two statements, allowing for more precise detection of confabulations. 

Formally, let \( D_k \) represent a decomposed summary unit (DSU) from summary \( S_i \), where \( k \) indexes the specific unit. The NLI model computes the entailment score \( E(D_k) \) for each DSU, where the score \( E(D_k) \) represents the probability distribution over entailment labels (entailment, neutral, contradiction).


\paragraph{Recursive Threshold-Based Text Segmentation (RTB-TS).} 

% Recursive Threshold-Based Text Segmentation (RTB-TS) is a novel technique we propose for further refining the granularity of summary content units beyond the sentence level, ensuring that each unit corresponds to an atomic fact. This method is crucial for accurately detecting and removing confabulated information, especially in complex, fact-dense biomedical summaries where traditional sentence-level segmentation might not be sufficient.
The algorithmic details of RTB-TS are described as follows:
\begin{itemize}
\item Initial Segmentation:
We begin by decomposing the summary \( S_i \) into DSUs \( D_k \) using a sentence boundary disambiguation technique:
$S_i \rightarrow \{D_1, D_2, \dots, D_k\}$.
This initial step provides a coarse segmentation based on sentence boundaries.

\item Pairwise NLI Scoring:
For each DSU \( D_k \), we compute the entailment score \( E(D_k) \) using a fine-tuned NLI model:
\begin{eqnarray}
E(D_k) &=& P(\text{entailment} \mid I, D_k),\\
N(D_k) &=& P(\text{neutral} \mid I, D_k),\\
C(D_k) &=& P(\text{contradiction} \mid I,  D_k).
\end{eqnarray}
Based on these scores, we classify the DSU as entailed, neutral, or contradictory.

\item Thresholding and Segmentation:
We apply a threshold to the entailment score to determine the initial classification:
\begin{eqnarray}
\text{Class}_\text{Entailed}(D_k) &=& E(D_k) > T_e,\\
\text{Class}_\text{Confab}(D_k) &=& N(D_k) + C(D_k) > T_c,\\
\text{Class}_\text{Uncertain}(D_k) &=& \text{otherwise},
\end{eqnarray}
where \( T_e \) is the entailment threshold and \( T_c \) is the confabulation threshold.
%
If \( D_k \) is classified as "uncertain," further segmentation is necessary.




\noindent

\item Recursive Decomposition:
For DSUs in the "uncertain" category, we recursively apply segmentation based on the identification of atomic facts within the DSU. This involves breaking down $D_k$ into finer sub-units $D_{k,a}$ where $a$ indexes each atomic fact:
$
D_k \rightarrow \{D_{k,1}, D_{k,2}, \dots, D_{k,a}\}
$.
%
We recompute the entailment score for each atomic fact sub-unit $D_{k,a}$:
\begin{eqnarray}
E(D_{k,a}) = P(\text{entailment} \mid I, D_{k,a}),
\end{eqnarray}
%
and retain only those atomic facts where the value of $E(D_{k,a})$ is greater than a chosen threshold.

\item Aggregation of Faithful DSUs:
After recursive segmentation and filtering, we aggregate the remaining faithful DSUs to form the refined summary:
\begin{eqnarray}
S_i^{\text{refined}} = \sum_k D_k^{\text{faithful}}.
\end{eqnarray}
The final refined summary \( S_i^{\text{refined}} \) should have suppressed the confabulated information.
%as h each unit corresponding to a verified atomic fact. 

%This stage prepares a refined summary which is free from confabulated information and prepares it for Stage 3, where any missing information identified due to overzealous confabulation removal is reintroduced, ensuring a balance between fidelity to the source text and comprehensiveness.
\end{itemize}


\subsection{Stage 3: Missing Information Addition (Comprehensiveness)}
%
Our summary should ideally encompass all the key information from the input document. To achieve this, we first identify the key sentences in the document and the key phrases in our summary. We then check whether all the key sentences are covered by the key phrases. If any key sentences are missing, we add them to the summary.
%
Unlike existing hybrid methods, such as~\cite{mao2020constrained}, which may produce initial summaries with confabulated information, our method separates the confabulation removal task (Stage 2) from the missing key information addition task (Stage 3). This approach minimizes the likelihood of introducing new confabulations in the final summary.

\paragraph{Key Information Extraction}
%
%Given a method for extracting key phrases~\cite{bennani2018simple,grootendorst2020keybert}
%
Our extracted key information from either the input document or our summary is described as follows. Let $K_{\rm doc} = \{ k_{\rm doc}^i \mid i \leq \rm top_M \}$ for the source document, and $K_{\rm summ} = \{ k_{\rm summ}^i \mid i \leq \rm top_N \}$ for the generated summary. Here, $K_{\rm doc}$ denotes a set of key sentences from the input document; $K_{\rm summ}$ refers to a set of the key phrases from our summary; $\rm top_M$ and $\rm top_N$ are the thresholds for the number of key sentences and key phrases, respectively.


For the input document, we use sentences as the minimum unit of granularity for extraction. For the summary generated in Stage 2, we apply a key phrase extraction method, such as~\cite{grootendorst2020keybert}, which extracts $n$-grams as key phrases. We then rank the sentences or phrases using $\rm MMR$~\cite{bennani2018simple} and select the top-$K$ as key sentences or key phrases, as shown in Algorithm~\ref{alg:1}.

\begin{algorithm}[t!]
\caption{Key Information Extraction}
\label{alg:1}
\begin{algorithmic}[1]
  \STATE ${\rm input} \gets  \text{document or summary}$
  \STATE $K \gets \{\}$
  \IF {$\rm input == \text{document}$} 
    \STATE ${\rm candidates} \gets \text{each sentence in document}$ 
  \ELSE
    \STATE ${\rm candidates} \gets \text{each phrase in summary}$ 
  \ENDIF
  \WHILE{${\rm len}(K) \leq {\rm topK}$}
    \STATE \[
      {\rm candidate}^* := \operatorname*{argmax}_{x \in {\rm candidates}} {\rm MMR(input, } K,  x)
    \]
    \STATE $ K \gets K + \rm candidate^*$
  \ENDWHILE
  \RETURN $K$
\end{algorithmic}
\end{algorithm}



\paragraph{Missing Key Information Detection}

Given $K_{\rm doc}$ and $K_{\rm summ}$, extracted from the source document and generated summary respectively, we calculate coverage scores ${\rm cov}_{\rm score}^{i}$ for each $k_{\rm doc}^i$ based on $K_{\rm summ}$. Specifically, we compute the embedding matrices for each key sentence and key phrase~\cite{reimers-2019-sentence-bert}:
%
\begin{eqnarray}
{\rm Embed}_{\rm doc} 
&=& \begin{bmatrix}
{\rm Encoder}(k_{\rm doc}^{1}) \\
\vdots \\
{\rm Encoder}(k_{\rm doc}^{m})
\end{bmatrix}_{m \times d}, \\
{\rm Embed}_{\rm summ} 
&=& \begin{bmatrix}
{\rm Encoder}(k_{\rm summ}^{1}) \\
\vdots \\
\rm Encoder(k_{\rm summ}^{n})]
\end{bmatrix}_{n \times d}.
\end{eqnarray}
%
%Similarity between the embedding matrices is computed using:
Similarities between $K_{\rm doc}$ and $K_{\rm summ}$ is computed using:
\begin{eqnarray}
[{\rm sim}^{i, j}]_{m \times n} = {\rm Embed}_{\rm doc} \cdot {\rm Embed}_{\rm summ}^{\rm T}.
\end{eqnarray}

The coverage scores of the key-sentences extracted from the input document in our summary is expressed as:
\begin{eqnarray}
{\rm Cov_{\rm score}} 
= \begin{bmatrix}
\max_{ j \leq n} \{{\rm sim}^{1, j}\} \\
\vdots \\
\max_{ j \leq n} \{{\rm sim}^{m, j}\}
\end{bmatrix}_{m \times 1}.
\end{eqnarray}
%
By defining ${\rm cov}^i_{\rm score} = \max_{ j \leq n} \{{\rm sim}^{i, j}\}$, we introduce a parameter ${\rm cov}_{\rm min}$, which represents the threshold for the coverage score. Any $k_{\rm doc}^{i}$ with a coverage score lower than ${\rm cov}_{\rm min}$ is considered missing information. Therefore, the potential missing information can be represented as:
\begin{eqnarray}
K_{\rm missing} = \{K_{\rm doc}^{i} \mid i \leq m, {\rm cov}_{\rm score}^{i} \leq {\rm cov}_{\rm min} \}.
\end{eqnarray}


\paragraph{Merging Missing Information to Summary}
With the extracted potential missing information $K_{\rm missing}$, the final step is to merge these into our summary one by one. Given $s$ sentences in the current summary, the potential locations to insert a single missing key sentence are denoted as ${\rm locs} = \{l \mid l \leq s + 1\}$.
%
We use perplexity ($\rm PPL$) to select the best location to insert a missing key sentence $k^i_{\rm missing} \in K_{\rm missing}$ into our summary~\cite{sharma2024textqualitybasedpruningefficient}:
\begin{eqnarray}
l^* = \operatorname*{argmin}_{l \in \rm locs} {\rm PPL}_{\rm LM}(k^i_{\rm missing}, {\rm summary},l ),
\end{eqnarray}
where ${\rm summary}$ is the current summary.
%
Since there may be several missing key sentences and the insertion process is dynamic, we employ a greedy algorithm, as shown in Algorithm~\ref{alg:2}. In this algorithm, $i$ represents the index of the missing key sentence to insert, and the function ${\rm insert}({\rm summ}_{\rm out}, {k}, l)$ represents the operation of inserting sentence $k$ after the $l$-th sentence in $\rm summ_{out}$.
%
\begin{algorithm}[t!]
\caption{Merge Missing Key Sentences to Summary}
\label{alg:2}
\begin{algorithmic}[1]
  \STATE ${\rm input} \gets $ \text{summary generated in Stage 2}
  \STATE $i \gets 0$
  \STATE $\rm summ_{out} \gets {\rm input}$
  \WHILE{$ i < {\rm topK}$}
    \STATE $s \gets$ number of sentences in $\rm summ_{out}$
    \STATE $locs := \{l \mid 0 \leq l \leq s\}$

    
    \STATE \(
      {l}^* := \operatorname*{argmin}_{l \in \rm locs} {\rm PPL}_{\rm LM}(k^i_{\rm missing}, {\rm summ}_{\rm out},l)
    \)
    
    \STATE ${\rm summ_{out}} \gets {\rm insert}({\rm summ_{out}}, k^i_{\rm missing}, l^*)$
    \STATE $i \gets i + 1$
  \ENDWHILE
  \RETURN $\rm summ_{out}$
\end{algorithmic}
\end{algorithm}



==> full_related_works.tex <==
\section{Related Work}

% \textcolor{red}{add hallu detection related work + issues in extractive (initial hallu summary) + Background and Assumptions part of each method section here - We should try to setup the issues each stage and the whole pipelines solves. We are missing related works for faithfulness and confabulation detection here.}

Summarization is usually approached by extractive and abstractive approaches~\cite{nenkova2011automatic,luo2024comprehensive}. 
Extractive summarization focuses on selecting key sentences or phrases directly from a document to create a summary. \citet{zhong2020extractive} treats it as a semantic text matching problem, matching the source document with candidate summaries in a shared space. \citet{sammet2023domain} utilizes BERT's contextual embeddings to enhance extraction of domain-specific terms, while \citet{song2023survey} highlights improvements in keyphrase extraction using pre-trained language models (PLMs). Although these methods enhance keyphrase identification, extractive summaries often suffer from verbosity and low fluency [cite].

Abstractive summarization, on the other hand, aims to rephrase content for more concise and readable summaries. \citet{wang2023element} uses element-aware test sets and a Summary Chain-of-Thought (SumCoT) approach to guide stepwise generation of summaries. \citet{chang2023booookscore} assess coherence in long document summarization, while \citet{roit2023factually} uses reinforcement learning to improve factual consistency. However, these models risk confabulations~\cite{maynez-etal-2020-faithfulness} and bias propagation \citet{ladhak2023pre}. %though techniques like those by~\citet{roit2023factually} can mitigate these issues.

% Extractive methods select key sentences or phrases from the input document to create a summary that retains the original wording. Meanwhile, abstractive methods rephrase the content to convey core ideas in new expressions. While research has focused on generic summarization, there is growing demand and increasing body of work concerning medical document summarization due to its critical importance.

% \paragraph{Extractive Summarization} 
% \citet{zhong2020extractive} treats the summarization task as a semantic text matching problem, allowing for a more holistic approach to selecting sentences from a source document. It matches the entire document with candidate summaries in a semantic space. 
% %
% \citet{sammet2023domain} leverages BERT's contextual embeddings to enhance the extraction of keywords tailored to specific domains. It utilizes BERT's ability to understand the nuances of language and thus captures domain-specific terminology and relationships.
% %
% % \citet{zhang2023extractive} assesses ChatGPT's performance in extractive summarization and compares it to traditional fine-tuning methods. It finds that, although ChatGPT scores lower on ROUGE metrics, it performs better on LLM-based evaluation metrics. It also introduces an extract-then-generate pipeline that leverages ChatGPT's strengths, leading to improved summary faithfulness.
% %
% Keyphrase extraction is key to extractive summarization.
% %
% %\cite{bennani2018simple} presents an unsupervised keyphrase extraction method that uses sentence embeddings, enabling real-time processing of large datasets and improving the diversity and coverage of extracted keyphrases.
% %
% \citet{song2023survey} offers a comprehensive review of advancements in keyphrase extraction techniques using pre-trained language models (PLMs), highlighting how PLMs enhance keyphrase extraction performance. \textcolor{magenta}{However, extractive summarisation has fundamental flaws. Direct extraction and aggregation of spans of keyphrases to generate the summary results in less fluent and overly verbose summaries.}
% %
% Constrained Abstractive Summarization (CAS)~\cite{mao2020constrained} provides a hybrid approach where by first generating an initial abstractive summary, then finding and adding in key missing information extractively. \textcolor{magenta}{While such hybrid methods which start with an abstractive summary  result in more readable and human preference aligned summaries, they still suffer from confabulations due to the abstractive generation of the initial summary.}


% %overall, while disparate attempts have been made to evaluate summarization methods with regard to their correctness and completeness  [something about, it hasn't been done comprehensively yet, let alone for the medical domain where they are key criteria]. Therefore, our work advances the state-of-the-art by [investigating where current approaches fail] and introducing a framework that jointly optimises [comprehensiveness and faithfulness]


% \paragraph{Abstractive Summarization}
% Compared to extractive summarization, abstractive summarization has received wider attention in recent years.
% %
% \cite{wang2023element} generates concise summaries by using expert-annotated element-aware test sets and employing a Summary Chain-of-Thought (SumCoT) technique, which guides LLMs to produce summaries step by step.
% %
% \cite{chang2023booookscore} investigates the challenges of summarizing long documents  using LLMs and introduces a novel automatic metric called BooookScore to evaluate the coherence of generated summaries. It examines two prompting workflows: hierarchical merging of chunk-level summaries and incremental updating of a running summary.
% %
% \cite{ladhak2023pre} explores how biases in pre-trained language models impact text summarization tasks. It finds that abstractive models allow biases to propagate more directly, resulting in hallucinated facts in summaries.
% %
% \cite{roit2023factually} addresses factual inconsistency in summaries using reinforcement learning with reference-free textual entailment rewards. This method improves summary faithfulness, salience, and conciseness, showing significant gains in both automatic and human evaluations. However, it may lead to less informative or more extractive summaries, potentially sacrificing detail.


% \paragraph{Medical Summarization}
% %
% %
% \cite{zhang2023famesumm} presents a framework aimed at enhancing the faithfulness of medical summaries generated by pre-trained language models through fine-tuning and contrastive learning techniques. By integrating medical knowledge and contextualizing medical terms, FaMeSumm achieves significant improvements in generating accurate and reliable summaries.
% %
% \cite{tang2023evaluating} examines the capabilities and limitations of LLMs in zero-shot medical evidence summarization. It also notes that automatic metrics often do not strongly correlate with summary quality.
% %
% \cite{ma2024iterative} leverages the in-context learning capability of ChatGPT to generate concise summaries of radiology reports by constructing dynamic prompts using semantically similar examples. 
% %
% \cite{ghosh2024clipsyntel} introduces a framework that combines CLIP and LLMs to create nuanced medical question summaries by integrating textual queries with visual representations of medical conditions. 
% %
% \cite{van2024adapted} shows that LLMs can outperform medical professionals in summarizing clinical texts, such as radiology reports and patient dialogues, by using adaptation methods to boost their performance.
% %
% \textcolor{magenta}{While this study benchmarks the impact of task adaptation such as QLlora and In Context Learning (ICL) in medical summarisation, there remains a lack of comprehensive benchmarks evaluating the efficacy of advanced summarization techniques (which better utilise model reasoning capabilities) in the biomedical domain. Additionally, such benchmarks often rely on inconsistent metrics for evaluation, which hampers the comparability of different approaches.}
\paragraph{Confabulated Information Detection.}
Confabulation detection, or the detection of information not grounded in the source text, is a significant challenge in medical summarization. Current work in this area typically focuses on providing a general factuality score to  evaluate a generated text \cite{maynez-etal-2020-faithfulness, liu2024hit, ji2023towards}, but this \textcolor{magenta}{does not address the need for systematic removal of confabulated spans of information from generated summaries.}  \citet{yadkori2024believe, manakul2023selfcheckgpt} use iterative prompting for probability amplification, combined with an information theoretic approach, while \citet{chen2024inside, farquhar2024detecting} use the model logit level information to find patterns which reduce epistemic uncertainty in models. However, these techniques only work in question/answering settings or cases situations where deterministic answer is expected, and cannot be easily extended to abstractive summarisation settings. Additionally, these techniques require access to the internal states of the model limiting their scalability and compatibility with proprietary models. \citet{maynez-etal-2020-faithfulness} find that traditional metrics often fail to align with human perceptions of faithfulness and factuality and concluding that entailment-based metrics are more accurate in reflecting human judgment. \citet{lei2023chain} also \textcolor{magenta}{demonstrate that entailment is a good candidate} for detecting hallucinated spans in summaries. \citet{ji2023towards} make use of LLM based self reflection for removing hallucinations in Medical QA tasks. However, removing confabulated spans from non deterministic generated texts such as summaries, remains an open task, with all techniques suffering from the common problem of overzealous removal of accurate information, leading to less fidelity.

Thus, there is a lack of a comprehensive study into \textcolor{magenta}{the impact of different advanced summarisation methods, as well as a complete framework for medical summarisation without confabulations and missing key information.}

%-- stanford paper, bioNLP, imageclef, ACI-bench (but not explicitly aiming for faithfulness). BioLaysum (but not aimed at domain experts). 





==> intro_first_2_paragraphs.tex <==
Large Language Models (LLMs) have demonstrated remarkable performance in various generative tasks, including zero-shot and out-of-the-box applications in specialized domains such as summarization~\cite{lei2023chain, van2024adapted}.
In the medical field, document summarization has emerged as a promising application, with the potential to significantly enhance the efficiency of medical staff in reviewing lengthy documents like patient histories or records.
% -- in medical domain, such assistance takes form in summarising long medical documents, as medical staff spends x time per day to .
% However, medical abstractive summarization presents a complex challenge, requiring a delicate balance between faithfulness and comprehensiveness.
%
% -- however, due to stochastic nature no formal guarantees, hence focus on assisting domain experts rather than automating their work
However, due to the stochastic nature and lack of formal guarantees arising from using LLMs for summarization~\cite{Li2023Team:PULSARModels,Schlegel2023PULSARRecords}, the generated summaries often deviate too much from the source documents, limiting their usability in real-world scenarios, especially in the medical domain where accurate and complete information is paramount for effective decision-making.
% maybe one sentence about how these are crucially important in medical domain, as introducing incorrect or omitting relevant information lowers the quality of evidence that decision-making doctors are presented with, ultimately resulting in false decisions which might impact patient outcomes.
For example, doctors rely on summaries that capture all relevant details without introducing any erroneous information.
These requirements directly translate to two critical aspects of medical summarization:
\emph{Faithfulness} and \emph{Informativeness}.
% \emph{Faithfulness} guarantees that the summary contains no hallucinations, factual errors, or confabulation where the generated text is not grounded in the source.
% On the other hand, \emph{Comprehensiveness} ensures that no vital information is omitted, and all the salient information (i.e., key phrases, entities, or relationships) present in the source document is necessarily included in the summary to provide complete information about the source document.
%
Summaries which are not \emph{faithful} or \emph{informative} can present doctors with incomplete or inaccurate evidence, potentially leading to misdiagnoses or inappropriate treatment decisions, ultimately impacting patient outcomes.

\textcolor{red}{Mention the novelty of the whole framework here - point out the issues of doing stage 2 and 3 in isolation - DONE here:}
In this paper, we present a unified framework addressing these two critical aspects of medical summarization.
Our approach enhances summary \emph{faithfulness} through confabulation removal and improves \emph{informativeness} via missing information addition.
Our work addresses a significant gap in recent summarization techniques, which typically tackle faithfulness and comprehensiveness in isolation, often failing to adequately address these crucial aspects in a unified manner.
More specifically, the lack of \emph{Faithfulness} leads to confabulation, where part of the summary contains information not present in the input document~\cite{maynez-etal-2020-faithfulness}.
Conversely, insufficient \emph{informativeness} results in relevant details missing from the input in the generated summary~\cite{mao2020constrained}.
In the domain of medical summarization, these two aspects are particularly crucial and must be addressed holistically.
Despite the critical nature of these requirements in the medical field, existing summarization approaches have not adequately prioritized or solved these challenges.
